Dynamic Flexibility Requests in Local Flexibility Markets: Quantifying the DSO Willingness to Pay

Local Flexibility Markets (LFMs) require Distribution System Operators (DSOs) to determine both the quantity of flexibility to procure and the corresponding willingness to pay during market clearing. Existing approaches typically rely on centralized AC-OPF clearing algorithms with limited practical scalability or strictly localized, static flexibility requests driven primarily by congestion management, while the economic value of flexibility is largely neglected. This paper proposes a dynamic flexibility-request methodology in which the DSO's willingness to pay is embedded directly into the market-clearing objective by monetizing transformer and cable aging, network losses, and voltage congestion. To enable computationally efficient clearing, exact convex piecewise-linear epigraph reformulations of the IEEE C57.91 transformer aging model and an Arrhenius-based cable aging model are developed and formally proven to preserve exactness. The proposed framework is validated on a modified CIGRE MV benchmark and compared with a recent state-of-the-art flexibility-request methodology. The results demonstrate significantly higher market liquidity, more efficient flexibility procurement, and improved network operations while preserving the market's transparency and non-discrimination principles.

==> Section_4.tex <==
\section{Case Study}
\label{sec:case_study}

\subsection{Network Model and Modifications}
\label{sec:cs_network}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/CIGRE.png}
    \caption{CIGRE single-line diagram of the studied 20-kV distribution system, including the primary and secondary substations.}
    \label{fig:cigre_network}
\end{figure}

The case study is built on the standard CIGRE European MV benchmark network. The original model represents a two-feeder meshed $110/20$~kV system with aggregated MV loads, although the network is operated radially, with the tie switches open. For the present study, the network is modified such that each controllable MV load point is represented by a dedicated $20/0.4$~kV secondary substation. Two MV buses, buses $1$ and $12$, are excluded from this secondary-substation expansion. These buses represent large, non-controllable MV demand points directly connected to the two primary feeders and remain fixed throughout the study. 

Following these modifications, the network contains two primary transformers and 14 secondary substations, as shown in Fig.~\ref{fig:cigre_network}. All simulations are performed over a $24$-hour horizon with hourly time steps. For the comparative analysis, the network-aware flexibility-request methodology of \cite{prat-network-aware} is implemented as a benchmark. Two spatial configurations are considered: bus-specific flexibility requests, where each controllable bus forms an individual flexibility zone, and the five-zone aggregation shown in Fig.~\ref{fig:cigre_network}, which groups multiple buses to increase the number of eligible providers and improve market liquidity.

\subsection{Operating Scenarios}
\label{sec:cs_scenarios}

Two operating scenarios are considered. The \textit{base case} represents a typical suburban load day. A common normalized \textit{duck-curve} active-load profile is applied identically to every load connected to the network. The \textit{stress case} retains the same duck-curve base demand but superimposes uncontrolled residential EV charging at each secondary substation. The EV load follows the statistical assumptions used in~\cite{11305421}. Each secondary substation serves $30-50$ customers based on their nominal apparent power, of which $30\%$ own an EV. Connection type is assigned probabilistically, with $80\%$ to three-phase supply and $20\%$ to single-phase supply. The corresponding home chargers are rated at $11$~kW (three-phase) and $7$~kW (single-phase). Each EV charges at its rated charger power until the daily trip energy is restored.

\subsection{Input Parameters}
\label{sec:cs_inputs}

\subsubsection{Transformer aging parameters}
The rated temperature rises are $\Delta\theta^{TO}_{R} = \SI{55}{\celsius}$ and $\Delta\theta^H_{R} = \SI{25}{\celsius}$. Oil and winding exponents are $n=m=0.8$; the top-oil and hotspot time constants are 3~h and 4~min, respectively. The normal life expectancy is taken as \SI{180000}{h}, and the replacement cost is assumed proportional to rated power at \SI{100000}{EUR/MVA}. The proposed piecewise-linear FAA approximates the Arrhenius curve over $[\SI{70}{\celsius},\SI{150}{\celsius}]$ with $80$ segments.

\subsubsection{Cable aging parameters}
The rated surface and core temperature rises are $\Delta\theta_{CS,R} = \SI{38}{\celsius}$ and $\Delta\theta_{C,R} = \SI{40}{\celsius}$, with time constants $\tau_{CS} = \SI{2}{h}$ and $\tau_C = \SI{0.0667}{h}$. The Arrhenius coefficient is $B = 15{,}000$, the normal cable life is \SI{438000}{h}, and the replacement cost is \SI{80000}{EUR/km} multiplied by the installed cable length. The proposed piecewise-linear FAA approximates the Arrhenius curve over $[\SI{40}{\celsius},\SI{120}{\celsius}]$ with $80$ segments.

\subsubsection{Assumptions}
For the LV loss, a uniform peak-loss ratio of $4\%$ is used for all secondary feeders. Voltage limits are enforced through soft penalties at $V_{\min} = 0.90$~p.u. and $V_{\max} = 1.10$~p.u., with willingness-to-pay values of \SI{10000}{EUR/pu} for both under- and over-voltage mitigation. 
This high violation penalty is adopted because, in the operational phase, congestion should be eliminated as much as possible. FSP bid formation is treated as exogenous and out of scope. For analysis purposes, hourly bid prices are randomly assigned within 60–90~EUR/MWh for 14 local providers (one per secondary substation), with capacities of 120~kW. These synthetic offers are used only to demonstrate the clearing mechanism and compare welfare outcomes; the proposed contribution lies in the DSO-side willingness-to-pay formulation, not in bidder modeling. 

For wholesale energy prices, the Cyprus day-ahead clearing price on 18~July~2026 is used \cite{TSOC_DAM_Prices}. For simplicity, only active-power flexibility is considered in the market-clearing formulation. Flexibility resources (e.g., battery energy storage systems) are assumed to modify their active-power injections or absorptions without changing their reactive-power set-points. Consequently, the baseline operating point is obtained from a full AC power-flow assuming a constant load power factor of 0.95, while reactive-power injections remain fixed throughout the optimization. If reactive-power flexibility directly or indirectly influences the operating point, the proposed framework can be readily extended by augmenting the sensitivity matrices and introducing the corresponding reactive-power decision variables. Such an extension is straightforward but falls outside the scope of this work, whose focus is the proposed DSO willingness-to-pay formulation.
